Historical Credibility for Movie Reviews and Its Application to Weakly Supervised Classification

In this study, we deal with the problem of judging the credibility of movie reviews. The problem is challenging because even experts cannot clearly and efficiently judge the credibility of a movie review and the number of movie reviews is very large. To tackle this problem, we propose historical credibility that judges the credibility of reviews based on the historical ratings and textual reviews written by each reviewer. For this, we present three kinds of criteria that can clearly classify the reviews into trusted or distrusted ones. We validate the effectiveness of the proposed historical credibility through extensive analysis. Specifically, we show that characteristics between the trusted or distrusted reviews are quite distinguishable in terms of three viewpoints: 1) distribution, 2) statistics, and 3) correlation. Then, we apply historical credibility to a weakly supervised model to classify a given review as a trusted or distrusted one. First, we show that it is significantly efficient because the entire data set is annotated according to the predefined criteria. Indeed, it can annotate 6,400 movie reviews only in 0.093 seconds, which occupy only 0.55%~1.88% of the total learning time when we use LSTM and SVM as the learning model. Second, we show that the historical credibility-based classification model clearly outperforms the textual review-based classification model. Specifically, the classification accuracy of the former outperforms that of the latter by up to 11.7%~13.4%. In addition, we clearly confirm that our classification model shows higher accuracy as the data size increases.

==> text/ch3-removed.tex <==
\section{Preliminaries}
\label{sec:sec3}

\subsection{Text representation models}
\label{sec:sec3-1}

In this paper, we build a learning model to classify movie reviews based on their credibility. To annotate movie reviews based on textual content, we need text representation models. We use two kinds of bag-of-words models: 1) TF-IDF and 2) Word2Vec. TF-IDF is a representative model for representing the text~\cite{jones2004statistical}. Word2Vec is a vector space model that embeds a corpus of text into a vector space~\cite{mikolov2013distributed}. The purpose of this paper is not to propose a specific novel text representation model. Instead, we choose some representative text representation models to show the effectiveness of the proposed learning method; we could equally apply any other models in place of TF-IDF and Word2Vec to the proposed method.

\subsubsection{TF-IDF}

TF-IDF represents the relative importance of words in a document based on the entire set of documents~\cite{wu2008interpreting}. Eq.~(\ref{equ1-1}) is the formula for obtaining TF-IDF, which is calculated by multiplying TF (text frequency) and IDF (inverse document frequency). Essentially, the result of TF-IDF increases as the frequency of given words in a document increases and the number of documents containing given words decreases. Eq.~(\ref{equ1-2}) and Eq.~(\ref{equ1-3}) are formulas for obtaining TF and IDF, respectively. TF is the frequency of a particular word in the document. Specifically, $f(i,j)$ is the frequency of a word $i$ in a document $j$ while $\max  \left\{ f(w,d):w\in d \right\}$ is the maximum of $f(i,j)$ of the words in the document. IDF is the total number of documents $|D|$ divided by the number of documents containing a word $t$. IDF uses a logarithm to prevent the result from increasing too much as $|D|$ increases~\cite{chowdhury2010introduction}. 

\begin{eqnarray}
\mathrm{TF-IDF_{i,j}} = TF_{i,j} \times IDF_{i}
\label{equ1-1}
\end{eqnarray}

\begin{eqnarray}
\mathrm{TF_{i, j}} = 0.5 + \frac{0.5 \times f(i, j)}{\max  \left\{ f(w,d):w\in d \right\} }
\label{equ1-2}
\end{eqnarray}

\begin{eqnarray}
\mathrm{IDF_{i}} =  \log\left( \frac{\mid D\mid}{count \left\{ d:t\in d  \right\}   }\right)
\label{equ1-3}
\end{eqnarray}

\subsubsection{Word2Vec}

Word2Vec is a word embedding model that maps words contained in the document into a vector space, where it tries to preserve contextual meanings~\cite{mikolov2013distributed}. Word2Vec supports two kinds of architectures~\cite{ling2015two}: 1) continuous bag-of-words~(simply, CBOW) and 2) continuous skip-gram, as shown in Fig.~\ref{fig:word2vec}. The continuous CBOW architecture tries to predict the center word from the context words. For example, in a given sentence, ``This movie \_ is wonderful,'' this architecture tries to find the most likely word to fill in the blank from the context. As a result, it shows better performance when we predict frequently used words. Conversely, the continuous skip-gram architecture tries to predict the context from a given center word. For example, for the given center word ``soundtrack,'' this architecture tries to predict the surrounding context.

\begin{figure}[!h]
\begin{subfigure}[b]{.47\linewidth}
  \centering
  \includegraphics[width=0.95\linewidth]{img/cbow.png}  
  \caption{Continuous bag-of-words~(CBOW)}
  \label{fig:cbox}
\end{subfigure}
\begin{subfigure}[b]{.48\linewidth}
  \centering
  \includegraphics[width=0.97\linewidth]{img/skipgram.png}  
  \caption{Continuous skip-gram}
  \label{fig:skipgram}
\end{subfigure}
\caption{Two architectures for Word2Vec~\cite{ling2015two}}
\label{fig:word2vec}
\end{figure}

\subsection{Machine learning techniques}
\label{sec:sec3-2}

For the classification of movie reviews, we apply machine learning techniques to the textual reviews. A variety of text classifiers using machine learning techniques have been proposed~\cite{ikonomakis2005text}: decision trees, naïve Bayes, rule induction, neural networks, nearest neighbors, and support vector machines~(SVMs). In this paper, we apply two techniques that have been studied for movie reviews~\cite{pang2002thumbs}: 1) naïve Bayes and 2) SVM. (As previously noted, we could apply any other machine learning techniques instead of naïve Bayes and SVM for the proposed method.)


\subsubsection{Naïve Bayes classifier} 

The naïve Bayes classifier has been widely used for document classification because it is quite simple but shows high accuracy~\cite{ch1997bayesian}. The name ``naïve Bayes’’ refers to a classifier based on Bayes' theorem. The important characteristic of the naïve Bayes classifier is that the features used for the classifier are stochastically independent of each other.

When a set of classes $C$ = \{${\mathbf c}_1$, ${\mathbf c}_2$, ..., ${\mathbf c}_n$\} is given, the naïve Bayes classifier predicts the ${\mathbf c}_i$ that is most likely to include a given document $d$ based on Bayes' theorem. Eq.~(\ref{equl-4}) shows Bayes' theorem, which gives the probability that a given document $d$ is included in a category ${\mathbf c}_i$. $P(d)$ is the probability of choosing a document $d$ from all the documents. $P$(${\mathbf c}_i$) is the number of documents in a category ${\mathbf c}_i$ divided by the total number of documents. $P$($d$\mid ${\mathbf c}_i$) is, for a given category ${\mathbf c}_i$, the probability of choosing document $d$ in that category. When a set of classes \{${\mathbf c}_1$, ${\mathbf c}_2$\} is given, we can predict the category in which a document $d$ is included by comparing $P$(${\mathbf c}_1\mid d$) and $P$(${\mathbf c}_2\mid d$).

\begin{eqnarray}
\mathrm{P(c_{i}\mid d)}=\frac{P(c_{i} ,d)}{P(d)} =  \frac{P(c_{i})P(d\mid c_{i})}{P(d)}
\label{equl-4}
\end{eqnarray}







\subsubsection{Support vector machines} 

A support vector machine~(SVM) finds the optimal hyperplane for a linear classification on data on a multidimensional space~\cite{vapnik2013nature}. Here, we can have multiple possible hyperplanes that can classify the data. The SVM finds a hyperplane having the maximal margin. Fig.~\ref{fig:fig3} shows an example of SVM-based classification. Here, when we compare candidate hyperplanes ${\mathbf B}_1$ and ${\mathbf B}_2$ in terms of the margin between the classified categories, ${\mathbf B}_1$ is chosen as the result hyperplane because its margin is greater than that of ${\mathbf B}_2$. The maximal margins concept aims to minimize incorrect classifications.

\begin{figure}[!h]
\centering{
\includegraphics[width=0.5\linewidth]{img/fig3_svm.png}
}
\caption{An example of the SVM classifier}
\label{fig:fig3}
\end{figure}

\begin{figure}[!h]
\begin{subfigure}[b]{.48\linewidth}
  \centering
  \includegraphics[width=0.95\linewidth]{img/fig4_a.png}  
  \caption{Linear classification}
  \label{fig:fig4-a}
\end{subfigure}
\begin{subfigure}[b]{.47\linewidth}
  \centering
  \includegraphics[width=0.95\linewidth]{img/fig4_b.png}  
  \caption{Nonlinear classification}
  \label{fig:fig4-b}
\end{subfigure}
\caption{The effect of nonlinear classification using a kernel function in SVM}
\label{fig:fig4}
\end{figure}


We can extend SVM to the case of nonlinear classification. For this, the kernel function has been introduced~\cite{wilk2016comparative}, defining additional functions for describing new dimensions required in nonlinear classification. Fig.~\ref{fig:fig4} shows the effect of nonlinear classification using the SVM kernel function. Fig.~\ref{fig:fig4-a} shows objects that are not classified by linear classification in SVM; Fig.~\ref{fig:fig4-b} shows that they can be classified by nonlinear classification using a kernel function. Kernel functions commonly used for the SVM classifier are the polynomial kernel, the Gaussian kernel, and the radial basis function~\cite{wilk2016comparative}.


\subsubsection{Semi-supervised support vector machines} 
\Red{As we mentioned earlier, SVM shows good classification performance in classification of multidimensional data by using kernel method.}
\Red{And, 이 장점에 기반한 Semi-supervised support vector machines~\cite{chapelle2005semi, bagattini2017simple, bagattini2017lagrangean}은 incomplete supervision의 Low-density separation method이다.}
\Red{Fig.~\ref{fig:s3vm}에서 확인할 수 있듯이 앞서 margin을 maximize하는 SVM boundary와 다르게 labeled data 뿐만 아니라 unlabeled data까지 포함된 전체 데이터에서 less dense한 방향을 찾아서 boundary가 형성된다.}
\Red{이 방법은 SVM을 사용할 수 있을 때 사용가능하며, optimization을 어떻게 할지에 관해서 연구들이 진행되고 있다~\cite{zhu2005semi}.}

\begin{figure}[!h]
\centering{
\includegraphics[width=0.5\linewidth]{img/fig3_s3vm.png}
}
\caption{An example of the S3VM classifier}
\label{fig:s3vm}
\end{figure}

